Matrix and Relative Weak Crossover in Japanese: An Experimental Investigation

This paper provides evidence that weak crossover effects differ in nature between matrix and relative clauses. Fukushima et al. (2024) provided similar evidence, showing that, when various non-structural factors were eliminated English speakers never accepted matrix weak crossover cases, but often accepted relative weak crossover ones. Those results were limited, however, by English word order, which lead to uncertainty as to whether this difference was due to the effects of linear precedence or syntactic structure. In this paper, to distinguish between these two possibilities, we conduct an experiment using Japanese, which lacks the word-order confound that English had. We find results that are qualitatively in line with Fukushima et al. (2024) suggesting that the relevant distinction is structural and not based simply on precedence.

==> figure/EBPHF-TypeCheck00.tex <==
\ensuremath{
  \Gamma, 
  u:\dSigmae[x]{
    \pred{boy}(x)
    }
  \turnstile{UDTT}
  \que: 
  \dSigma[x]{\Entity}{
    \pred{male}(x)
    }
}

==> figure/EBPHF-ccg.tex <==
\ph[>]{
  S
  }{
  \ph[>]{
    \vT/(\vT\bs\np)
    }{
    \clex{Every}{\vT/(\vT\bs\np)/N}
    &
    \clex{boy}{N}
    }
  &
  \ph[<]{
    S\bs\np
    }{
    \clex{loves}{S\bs\np/\np}
    &
    \ph[>]{
      \vT\bs(\vT/\np)
      }{
      \clex{his}{\vT\bs(\vT/\np)/(N\bs\np)}
      &
      \clex{mother}{N\bs\np}
      }
    }
  }


==> figure/EBPHF-sem.tex <==
\ensuremath{
  \dPi[u]{
    \dSigmae[x]{
      \pred{boy}(x)
      }
    }{
    \begin{dBox}
    \dAsp[w]{
      \dSigmae[z]{
        \pred{male}(z)
        }
      } \\
    \dAsp[v]{
      \begin{dBox}
      y:\Entity \\
      \pred{motherOf}(y,\pi_1w)
      \end{dBox}
      } \\
    \pred{love}(\pi_1u,\pi_1v)
    \end{dBox}
    }
}

==> figure/HFPEB-TypeCheck00.tex <==
\ensuremath{
  \Gamma
  \turnstile{UDTT}
  \que: \dSigma[x]{\Entity}{
    \pred{male}(x)
    }
}

==> figure/HFPEB-ccg.tex <==
\ph[>]{
  S
  }{
  \ph[>]{
    \vT/(\vT\bs\np)
    }{
    \clex{his}{\vT/(\vT\bs\np)/(N\bs\np)}
    &
    \clex{mother}{N\bs\np}
    }
  &
  \ph[<]{
    S\bs\np
    }{
    \clex{loves}{S\bs\np/\np}
    &
    \ph[>]{
      \vT\bs(\vT/\np)
      }{
      \clex{every}{\vT\bs(\vT/\np)/N}
      &
      \clex{boy}{N}
      }
    }
  }


==> figure/HFPEB-sem.tex <==
\ensuremath{
    \begin{dBox}
    \dAsp[w]{
      \dSigmae[z]{
        \pred{male}(z)
        }
      } \\
    \dAsp[v]{
      \begin{dBox}
      y:\Entity \\
      \pred{motherOf}(y,\pi_1w)
      \end{dBox}
      } \\
    \dPi[u]{
      \dSigmae[x]{
        \pred{boy}(x)
        }
      }{
      \pred{love}(\pi_1u,\pi_1v)
      }
    \end{dBox}
}

==> figure/MMaBwHFP-TypeCheck00.tex <==
\ensuremath{
  \Gamma,\ 
  x:\Entity,\ 
  b:\pred{boy}(x)\ 
  \turnstile{UDTT}
  \que: 
  \dSigma[x]{\Entity}{
    \pred{male}(x)
    }
}

==> figure/MMaBwHFP-ccg.tex <==
\ph[>]{
  S
  }{
    \ph[>]{
      \vT/(\vT\bs\np)
      }{
      \clex{every}{\vT/(\vT\bs\np)/N}
      &
      \ph[<]{
        N
        }{
        \clex{boy}{N}
        &
        \ph[>]{
          N \bs N
          }{
          \clex{who}{N\bs N/(S/\np)}
          &
          \clex{his mother loves}{S/\np}
          }
        }
      }
  &
  \ph[<]{
    S\bs\np
    }{
    \clex{bought}{S\bs\np/\np}
    &
    \clex{flowers}{\vT/(\vT\bs\np)}
    }
  }


==> figure/MMaBwHFP-sem.tex <==
\ensuremath{
  \dPi[u]{
    \dSigmae[x]{
    b:\pred{boy}(x) \\
    \dAsp[w]{
      \dSigmae[z]{
        \pred{male}(z)
        } 
      } \\
    \dAsp[v]{
      \begin{dBox}
      y:\Entity \\
      \pred{motherOf}(y,\pi_1w)
      \end{dBox}
      } \\
    \pred{love}(\pi_1v,x)
    }
    }{
    \pred{buy}(\pi_1u,\name{f})
    }
}

==> figure/MMaBwPHF-ccg.tex <==
\ph[>]{
  S
  }{
    \ph[>]{
      \vT/(\vT\bs\np)
      }{
      \clex{every}{\vT/(\vT\bs\np)/N}
      &
      \ph[<]{
        N
        }{
        \clex{boy}{N}
        &
        \ph[>]{
          N \bs N
          }{
          \clex{who}{N\bs N/(S\bs\np)}
          &
          \clex{loves his mother}{S\bs\np}
          }
        }
      }
  &
  \ph[<]{
    S\bs\np
    }{
    \clex{bought}{S\bs\np/\np}
    &
    \clex{flowers}{\vT/(\vT\bs\np)}
    }
  }


==> figure/MMaBwPHF-sem.tex <==
\ensuremath{
  \dPi[u]{
    \dSigmae[x]{
    b:\pred{boy}(x) \\
    \dAsp[w]{
      \dSigmae[z]{
        \pred{male}(z)
        } 
      } \\
    \dAsp[v]{
      \begin{dBox}
      y:\Entity \\
      \pred{motherOf}(y,\pi_1w)
      \end{dBox}
      } \\
    \pred{love}(x,\pi_1v)
    }
    }{
    \pred{buy}(\pi_1u,\name{f})
    }
}

==> figure/lexicon.tex <==
\lexsem{every}{\vT/(\vT\bs\np),\vT\bs(\vT/\np)}{\LAM[n]\LAM[p]\LAM[\vec{x}]\dPi[u]{\dSigmae{n(x)}}{p\vec{x}(\pi_1u)}} \\
\lexsem{boy}{N}{\LAM[x]\pred{boy}(x)} \\
\lexsem{loves}{S\bs\np/\np}{\LAM[y]\LAM[x]\pred{love}(x,y)} \\
\lexsem{his}{\vT\bs(\vT/\np)/(N\bs\np)}{
        \LAM[r]\LAM[p]\LAM[\vec{x}]\begin{dBox}
        \dAsp[u]{
          \dSigma[x]{\Entity}{
            \pred{male}(x)
            }
          } \\
        \dAsp[v]{
          \begin{dBox}
          y:\Entity \\
          r(y)(\pi_1u)
          \end{dBox}
          } \\
        p\vec{x}(\pi_1v)
        \end{dBox}
  } \\
\lexsem{mother}{N\bs\np}{\LAM[z]\LAM[y]\pred{motherOf}(y,z)} \\
\lexsem{who}{N\bs N/(S\bs\np), N\bs N/(S/\np)}{
  \LAM[p]\LAM[n]\LAM[x] \dConj{nx}{px}
  } \\
\lexsem{bought}{S\bs\np/\np}{\LAM[y]\LAM[x]\pred{buy}(x,y)} \\
\lexsem{flowers}{\vT/(\vT\bs\np)}{\LAM[p]p(\name{f})} \\

